Fairness Degrading Adversarial Attacks Against Clustering Algorithms

Clustering algorithms are ubiquitous in modern data science pipelines, and are utilized in numerous fields ranging from biology to facility location. Due to their widespread use, especially in societal resource allocation problems, recent research has aimed at making clustering algorithms fair, with great success. Furthermore, it has also been shown that clustering algorithms, much like other machine learning algorithms, are susceptible to adversarial attacks where a malicious entity seeks to subvert the performance of the learning algorithm. However, despite these known vulnerabilities, there has been no research undertaken that investigates fairness degrading adversarial attacks for clustering. We seek to bridge this gap by formulating a generalized attack optimization problem aimed at worsening the group-level fairness of centroid-based clustering algorithms. As a first step, we propose a fairness degrading attack algorithm for k-median clustering that operates under a whitebox threat model -- where the clustering algorithm, fairness notion, and the input dataset are known to the adversary. We provide empirical results as well as theoretical analysis for our simple attack algorithm, and find that the addition of the generated adversarial samples can lead to significantly lower fairness values. In this manner, we aim to motivate fairness degrading adversarial attacks as a direction for future research in fair clustering.

==> discussion.tex <==
\looseness-1 A major limitation of our work is running time. We present empirical results in the appendix (Section E). While not prohibitively slow, in comparison to fair clustering algorithms, Algorithm 1 is generally slower and requires careful parameterization for convergence. Similar limitations hold for the other algorithms. However, we believe that despite these shortcomings, our paper opens up an important alternative direction for future research in fair clustering, as our experiments also demonstrate. 

%-- for example, the first work on fair clustering \citep{chierichetti2017fair} did not scale well with data and could only accommodate 2 protected groups, and yet lead to many papers with subsequent improvements.
%%, with Algorithm 3 incurring the extra overhead of the process used to find fair centers.

==> related_works.tex <==
\iffalse
Researchers have recently studied clustering algorithms with fairness guarantees, or proposed fair variants to existing clustering algorithms. Most of this work has looked at center-based clustering (such as k-means, and k-median) \citep{bercea2018cost}, \citep{chierichetti2017fair}, \citep{backurs2019scalable}, \citep{bera2019fair}, \citep{chen2019proportionally}, \citep{schmidt2018fair}, \citep{ziko2019clustering}, and more recently, spectral methods \citep{kleindessner2019guarantees}, \citep{anagnostopoulos2019principal}. This line of work seeks to impose some \textit{fairness} constraints along with the original clustering objective. Then the goal is to provide algorithms that approximate this fair objective. Fair algorithmic variants for the k-center and k-median clustering objectives were first proposed by \citep{chierichetti2017fair}. Many works have followed that improve upon these ideas, either in terms of approximation rates \citep{backurs2019scalable}, \citep{bercea2018cost}, allowing for multiple protected groups \citep{bercea2018cost}, \citep{rosner2018privacy}, extending it to other clustering objectives \citep{kleindessner2019guarantees}, \citep{schmidt2018fair}, or a combination of these, among others. Some works also look at alternate notions of fairness for center-based clustering \citep{chen2019proportionally} \citep{ghadiri2020fair}. Interestingly, the formulation of the antidote data problem for clustering also has connections to \textit{machine teaching} \citep{zhu2018overview}, where the upper-level problem defines the teacher's cost, and the clustering problem is the victim/learner. Furthermore, the concept of adding antidote data to improve fairness was first proposed by \citep{rastegarpanah2019fighting} for recommendation systems, so our work is thematically similar to theirs as well.
\fi


%\iffalse
\looseness-1 \textbf{Fairness in Machine Learning.} ML algorithms can be made \textit{fair} in three stages of the learning pipeline \citep{caton2020fairness, mehrabi2019survey}-- \textit{before-training} (pre-processing the dataset), \textit{during-training} (changing the ML algorithm), or \textit{after-training} (post-processing the learnt model). Most research on fair clustering focuses on the \textit{during-training} phase \citep{bera2019fair, bercea2018cost, backurs2019scalable, chierichetti2017fair, schmidt2018fair, ziko2019clustering, kleindessner2019guarantees, ghadiri2020fair} and proposes fair clustering algorithms. In their paper, \citep{davidsonmaking} study the \textit{after-training} phase for improving fairness post-clustering. The approaches proposed in our paper are novel since they improve fairness for clustering models in the \textit{before-training} stage. Further, our approaches can accommodate general fairness notions and clustering algorithms. %Another consideration is the fairness notion being employed which varies depending on application context and type of ML model used. In contrast, our approaches can accommodate general fairness notions and clustering algorithms.

\textbf{Machine Teaching.} Our approach in this paper is inspired by the techniques in \textit{machine teaching} literature~\citep{goldman1995complexity,doliwa2014recursive,DBLP:conf/icml/SinglaBBKK14,zhu2015machine,zhu2018overview,DBLP:conf/nips/ChenSAPY18,DBLP:conf/nips/PeltolaCDK19}. Machine teaching studies the interaction between a teacher and a learner where the teacher selects training examples for the learner to learn a specific task. A machine teaching problem can be cast in a bi-level form where the upper-level problem defines the teacher's cost and the lower-level problem defines the learner's method. Variations of this bi-level form can be used to formulate teacher's optimization problem in a variety of learning settings, including supervised learning~\citep{zhu2013machine,liu2016teaching,DBLP:conf/nips/Mansouri0VZS19,DBLP:conf/ijcai/DevidzeMH0S20}, imitation learning~\citep{cakmak2012algorithmic,DBLP:conf/nips/HaugTS18,DBLP:conf/ijcai/KamalarubanDCS19,brown2019machine,DBLP:conf/nips/TschiatschekGHD19}, and reinforcement learning~\citep{DBLP:conf/aaai/ZhangP08,DBLP:conf/sigecom/ZhangPC09,DBLP:conf/icml/RakhshaRD0S20,DBLP:conf/nips/MaZSZ19,DBLP:journals/corr/abs-2011-10824}. In the proposed antidote data problem for clustering, the upper-level problem (teacher's cost) is the cost of adding antidote data, and the lower-level problem (learner) is the clustering algorithm. 

%In its basic form, the formulation of machine teaching focusses The teacher aims to \textit{teach} a specific model to the student, while minimizing the teaching cost. 
%

%Our work also has connections to \textit{machine teaching} \citep{zhu2018overview}, where problems are formulated in a bi-level form. The upper-level problem defines the teacher's cost, and the lower-level problem is the learner. The teacher aims to \textit{teach} a specific model to the student, while minimizing the teaching cost. Machine teaching has been extensively studied for supervised learning \citep{kumar2020average, kumar2021teaching} and reinforcement learning \citep{rakhsha2020policy}, \citep{NEURIPS2019_3de568f8}. In the proposed antidote data problem for clustering, the upper-level problem (teacher's cost) is the cost of adding antidote data, and the lower-level problem (learner) is the clustering algorithm. 


\looseness-1 \textbf{Bi-level Optimization.} Bi-level problems involve a two-level hierarchical optimization. For these, a lower-level problem exists, which influences the solutions for an upper-level problem. Both bi-level optimization and verifying the optimality of an obtained solution are NP-Hard \citep{bilevelnp, bilevelnp2}. This makes finding optimal solutions and evaluating them non-trivial tasks. In the paper, the main problem considered is a complex bi-level optimization, where both upper-level and lower-level problems can be non-convex optimization problems. Many techniques for bi-level programming exist, but most of these assume simple forms for the upper/lower problems, or use evolutionary methods for which theoretical results are hard to provide \citep{sinha2017review}. Despite these challenges, we provide algorithms that obtain feasible solutions to the bi-level problem and outperform state-of-the-art fair clustering approaches.



%\fi

==> results.tex <==

\iffalse
\subsection{Datasets used}

1. \underline{\texttt{adult} \citep{kohavi1996scaling}}. The UCI \textit{adult} dataset consists of 10000 samples with 5 features (\textit{age, education-num, final-weight, capital-gain, hours-per-week}) chosen for clustering. The original dataset contains 48842 samples, but like previous works \citep{chierichetti2017fair}, \citep{abraham2019fairness} we remove missing values and undersample to 10000 samples. The protected groups are \textit{white, black, asian-pac-islander, amer-indian-eskimo, other} signifying the feature \textit{race}. Therefore, $n \times d = 10000 \times 5$.
    
2. \underline{\texttt{bank} \citep{moro2014data}}. The UCI \texttt{bank} dataset contains 45211 samples and 3 features (\textit{age, balance, duration}), i.e. $n \times d = 45211 \times 3$. The protected groups for \texttt{bank} are \textit{married, single, divorced} signifying \textit{marital status}.
    
3. \underline{\texttt{creditcard} \citep{yeh2009comparisons}}. The UCI \texttt{creditcard} data comprises of 30000 samples ($n$) with 23 features ($d$). The protected groups are \textit{higher} and \textit{lower} education signifying the feature \textit{education}.

4. \underline{\texttt{LFW} \citep{huang2008labeled}}. The Labeled Faces in the Wild dataset (\texttt{LFW}) contains 13232 celebrity images ($n$) with each image of dimension $49 \times 36 = 1764$ features. The protected groups are \textit{male, female} signifying the feature \textit{sex}. As is common with clustering on image datasets \citep{ghadiri2020fair}, we also project from $1764$ features to $80$ features ($d$) via PCA.
\fi


We consider four real-world datasets commonly used to evaluate fair clustering algorithms: \texttt{adult} \citep{kohavi1996scaling}, \texttt{bank} \citep{moro2014data}, \texttt{creditcard} \citep{yeh2009comparisons}, and Labeled Faces in the Wild (\texttt{LFW}) \citep{huang2008labeled}. The \texttt{adult} dataset has $10000 \times 5$ samples, and protected groups signify \textit{race} (\textit{white, black, asian-pac-islander, amer-indian-eskimo, other}). The \texttt{bank} dataset has $45211 \times 3$ samples, and protected groups signify \textit{marital status} (\textit{married, single, divorced}). The \texttt{creditcard} dataset has $30000 \times 23$ samples, and the protected groups signify \textit{education} (\textit{higher} and \textit{lower} education). \texttt{LFW} has $13232 \times 80$ samples, and the protected groups signify \textit{sex} (\textit{male, female}). 

\looseness-1 We next provide results obtained for Algorithm 1 and Algorithm 3 on the aforementioned datasets. We defer the results for Algorithm 2 (with $\mathcal{C}_{\textrm{SON}}$ and $\mathcal{F}_{\textrm{social}}$) to the appendix (Section C) as we are solving a convex problem for which the results can be obtained in a straightforward manner.

\subsection{Results for Algorithm 1}
 \looseness-1 For Algorithm 1 we present results for $\mathcal{C}_{\textrm{k-medoids}}$ and $\mathcal{F}_{\textrm{social}}$ ($\mathcal{F}$ can be arbitrary). We first obtain $\mu^{\dagger}$ by running the Fair-Lloyd algorithm of \citep{ghadiri2020fair} and then project centers to the set $U$ as they have to be medoids. The original centers obtained by clustering on just $U$ are denoted as $\mu^0$. Using Algorithm 1 we aim to compute $V$ such that the centers obtained by clustering on $U\cup V$ are the target center set. That is, through Algorithm 1, we aim to reduce the initial distance between centers given by $||\mu^0 - \mu^{\dagger}||_F$. We vary $k$ from 2 to 4, and run Algorithm 1 on all 4 datasets with $\epsilon = 0, \xi = 1$. The results are shown in Table 1. As can be seen, by clustering on $U\cup V$, the obtained centers $\mu$ are now exactly the target center set $\mu^{\dagger}$, ie $||\mu - \mu^{\dagger}||_F = 0$. As $\mathcal{F}_{\textrm{social}}(\mu^{\dagger}, U) \leq \alpha$, we have $\mathcal{F}_{\textrm{social}}(\mu, U) \leq \alpha$. Thus, Algorithm 1 effectively achieves the goal of meeting the fairness constraint while adding a minimal number of antidote data points. Results for k-means are present in the appendix (Section B.1).

\vspace{-0.35cm}

\begin{table}[ht!]
\centering
\fontsize{7}{7}\selectfont
\caption{Results for Algorithm 1 with $\mathcal{C}_{\textrm{k-medoids}}$ and $\mathcal{F}_{\textrm{social}}$. (Consider $k=2$ and the \texttt{LFW} dataset as an example. The distance between the original centers $\mu^0$ and target fair centers $\mu^{\dagger}$ is $||\mu^0 - \mu^{\dagger}|| = $ 28.418. The fairness cost for $\mu^0$ is $\mathcal{F}_{\textrm{social}}(\mu^0, U) = $ 1631.385 and for $\mu^{\dagger}$ is $\mathcal{F}_{\textrm{social}}(\mu^{\dagger}, U) = $ 1532.679. After Algorithm 1 is run, $V$ is obtained, with size $|V| = $ 0.0757$|U|$, indicating minimal antidote data addition. Cluster centers $\mu$ obtained by clustering on $U\cup V$ are now $\mu^{\dagger}$ as $||\mu - \mu^{\dagger}|| = 0$. The fairness constraint has been met. Refer to Section 4.1.)}
\begin{tabular}{cc||ccc||cc}
\hline
\#Clusters & Dataset & $||\mu^0 - \mu^{\dagger}||$ & $\mathcal{F}_{\textrm{social}}(\mu^0, U)$ & $\mathcal{F}_{\textrm{social}}(\mu^{\dagger}, U)$ & $|V|/|U|$ & $||\mu - \mu^{\dagger}||$ \\ \hline%\hline
\multirow{4}{*}{$k = 2$} & \texttt{adult} & 14.427 & 5.559 & 4.224 & 0.0075 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{bank} & 0.239 & 2.343 & 2.313 & 0.0112 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{creditcard} & 2.276 & 21.387 & 21.151 & 0.0068 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{LFW} & 28.418 & 1631.385 & 1532.679 & 0.0757 & \textbf{0.0} \\ \hline
\multirow{4}{*}{$k = 3$} & \texttt{adult} & 0.966 & 3.609 & 3.572 & 0.01 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{bank} & 0.294 & 1.802 & 1.781 & 0.0487 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{creditcard} & 4.047 & 18.771 & 18.727 & 0.01 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{LFW} & 55.3336 & 1532.592 & 1476.691 & 0.144 & \textbf{0.0} \\ \hline
\multirow{4}{*}{$k=4$} & \texttt{adult} & 2.164 & 3.120 & 2.942 & 0.07 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{bank} & 0.241 & 1.322 & 1.295 & 0.0155 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{creditcard} & 12.357 & 19.486 & 17.077 & 0.01 & \textbf{0.0} \\ %\cline{2-7} 
 & \texttt{LFW} & 66.426 & 1466.232 & 1399.454 & 0.0832 & \textbf{0.0} \\ \hline
\end{tabular}
\end{table}

\subsection{Results for Algorithm 3}
\looseness-1 We compare Algorithm 3 against vanilla clustering and state-of-the-art fair clustering algorithms. Throughout we let $k=2$ and due to space limitations, present results for $k=3$ and $k=4$ in the appendix (Section D.1). We also compare Algorithm 3 and other fair clustering approaches in terms of clustering performance, using clustering performance metrics such as the Silhouette coefficient \citep{ROUSSEEUW198753}, Calinski-Harabasz score \citep{chindex}, and the Davies-Bouldin index \citep{dbindex}. We use these metrics to unify comparisons across the different clustering algorithms considered in experiments. For all experiments, we choose $\alpha$ to be the fairness cost of the algorithms being compared against (vanilla clustering, fair algorithms) so as to improve on them. We let $\mathcal{A}$ be the \texttt{RACOS} \citep{racos} algorithm, $V_s = 10, n' = 100, \xi = 1$.


\looseness-1 \textbf{Comparing Algorithm 3 With Vanilla Clustering and Fair Clustering Approaches}. Since Algorithm 3 can accommodate general $\mathcal{C}$ and $\mathcal{F}$, we experiment on 3 combinations: Combination \#1 with $\mathcal{C}_{\textrm{k-means}}$ and $\mathcal{F}_{\textrm{social}}$, Combination \#2 with $\mathcal{C}_{\textrm{k-means}}$ and $\mathcal{F}_{\textrm{social}}$, and Combination \#3 where $\mathcal{C}$ is unnormalized spectral clustering, and $\mathcal{F}$ is $\mathcal{F}_{\textrm{balance}}$. The results when comparing against vanilla clustering are shown in Table 2. Vanilla cluster centers are denoted as $\mu^{\textrm{vanilla}}$ and centers obtained via Algorithm 3 are denoted by $\mu$. As can be seen we add very few antidote data points ($|V|/|U|$) and improve on the fairness cost over vanilla clustering. For each of the combination settings considered, we also compare against an equivalent state-of-the-art fair clustering algorithm. For Combination \#1 we consider the algorithm of Bera et al \citep{bera2019fair}, for Combination \#2 we consider the Fair-Lloyd algorithm of Ghadiri et al \citep{ghadiri2020fair}, and for Combination \#3 we consider the algorithm of Kleindessner et al \citep{kleindessner2019guarantees}. Since the approach of \citep{kleindessner2019guarantees} cannot handle large datasets, we subsample each dataset to 1000 samples for Combination \#3. The results are shown in Table 3, and centers obtained from fair clustering algorithms are denoted as $\mu^{\textrm{SOTA}}$. We find that we outperform fair algorithms in terms of lower fairness costs. 

%\vspace{-0.11cm}


% 1 indicating a well-defined clustering and -1 indicating ill-formed clusters
%\vspace{-0.2cm}


%\vspace{-0.2cm}

\begin{table*}[ht!]
\fontsize{7}{7}\selectfont %8
\caption{Comparing fairness costs of Algorithm 3 with vanilla clustering. (Consider Combination \#1 and the \texttt{bank} dataset as an example. The fairness cost for the vanilla cluster centers $\mu^{\textrm{vanilla}}$ is $\mathcal{F}(\mu^{\textrm{vanilla}}, U) = -\textrm{0.3054}$ and $\alpha$ is set to this value to improve on this fairness cost. After Algorithm 3 is run, $V$ is obtained, with size $|V| = $ 0.00011$|U|$. Cluster centers $\mu$ obtained by clustering on $U\cup V$ result in fairness cost $\mathcal{F}(\mu, U) = -\textrm{0.3077}$. This is lower than $\mathcal{F}(\mu^{\textrm{vanilla}}, U)$, leading to improved fairness. Refer to Section 4.2 for more details.)}
\centering
\begin{tabular}{cc||cc||cc}
\hline
Clustering-Fairness Combination & Dataset & $\alpha$ & $|V|/|U|$ & $\mathcal{F}(\mu^{\textrm{vanilla}}, U)$ & $\mathcal{F}(\mu, U)$ \\ \hline%\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Combination \#1:\\ $\mathcal{C}_{\textrm{k-means}}, \mathcal{F}_{\textrm{balance}}$\end{tabular}} & \texttt{adult} & -0.6119 & 0.001 & -0.6119 & \textbf{-0.6196} \\
 & \texttt{bank} & -0.3054 & 0.00011 & -0.3054 & \textbf{-0.3077} \\
 & \texttt{creditcard} & -0.8696 & 0.00017 & -0.8696 & \textbf{-0.8715} \\
 & \texttt{LFW} & -0.8815 & 0.00075 & -0.8815 & \textbf{-0.8821} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Combination \#2:\\ $\mathcal{C}_{\textrm{k-means}}, \mathcal{F}_{\textrm{social}}$\end{tabular}} & \texttt{adult} & 5.3678 & 0.0005 & 5.3678 & \textbf{4.2104} \\
 & \texttt{bank} & 2.3432 & 0.00022 & 2.3432 & \textbf{2.3416} \\
 & \texttt{creditcard} & 19.740 & 0.00034 & 19.740 & \textbf{19.729} \\
 & \texttt{LFW} & 1406.3411 & 0.00076 & 1406.3411 & \textbf{1406.1676} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Combination \#3:\\ $\mathcal{C}_{\textrm{spectral}}, \mathcal{F}_{\textrm{balance}}$\end{tabular}} & \texttt{adult} & -0.6458 & 0.001 & -0.6458 & \textbf{-0.6911} \\
 & \texttt{bank} & -0.4811 & 0.00022 & -0.4811 & \textbf{-0.5489} \\
 & \texttt{creditcard} & -0.8384 & 0.00034 & -0.8384 & \textbf{-0.8407} \\
 & \texttt{LFW} & -0.9279 & 0.00076 & -0.9279 & \textbf{-0.9389} \\ \hline
\end{tabular}
\end{table*}


\begin{table*}[ht!]
\fontsize{7}{7}\selectfont %8
\caption{Comparing fairness costs of Algorithm 3 with fair clustering algorithms. (Reads similarly to Table 2.)}%This table reads similarly to Table 2. The cluster centers obtained via the state-of-the-art fair clustering algorithm are $\mu^{\textrm{SOTA}}$ and Algorithm 3 obtains centers $\mu$ with fairness cost $\mathcal{F}(\mu, U) < \mathcal{F}(\mu^{\textrm{SOTA}}, U)$. Refer to Section 4.2 for more details.)}
\centering
\begin{tabular}{cc||cc||cc}
\hline
Clustering-Fairness Combination & Dataset & $\alpha$ & $|V|/|U|$ & $\mathcal{F}(\mu^{\textrm{SOTA}}, U)$ & $\mathcal{F}(\mu, U)$ \\ \hline%\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Combination \#1:\\ $\mathcal{C}_{\textrm{k-means}}, \mathcal{F}_{\textrm{balance}}$\end{tabular}} & \texttt{adult} & -0.6059 & 0.001 & -0.6059 & \textbf{-0.6196} \\
 & \texttt{bank} & -0.3065 & 0.00011 & -0.3065 & \textbf{-0.3077} \\
 & \texttt{creditcard} & -0.8696 & 0.00017 & -0.8696 & \textbf{-0.8715} \\
 & \texttt{LFW} & -0.8816 & 0.00075 & -0.8816 & \textbf{-0.8821} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Combination \#2:\\ $\mathcal{C}_{\textrm{k-means}}, \mathcal{F}_{\textrm{social}}$\end{tabular}} & \texttt{adult} & 4.2636 & 0.0005 & 4.2636 & \textbf{4.2104} \\
 & \texttt{bank} & 2.3135 & 0.1549 & 2.3135 & \textbf{2.3119} \\
 & \texttt{creditcard} & 18.998 & 0.19 & \textbf{18.998} & \textbf{18.998} \\
 & \texttt{LFW} & 1344.5468 & 0.3999 & 1344.5468 & \textbf{1344.5461} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Combination \#3:\\ $\mathcal{C}_{\textrm{spectral}}, \mathcal{F}_{\textrm{balance}}$\end{tabular}} & \texttt{adult} & -0.5973 & 0.001 & -0.5973 & \textbf{-0.6911} \\
 & \texttt{bank} & -0.6086 & 0.5 & -0.6086 & \textbf{-0.6899} \\
 & \texttt{creditcard} & -0.8407 & 0.38 & -0.8407 & \textbf{-0.9990} \\
 & \texttt{LFW} & -0.9926 & 0.4 & -0.9926 & \textbf{-0.9997} \\ \hline
\end{tabular}
\end{table*}

\looseness-1 \textbf{Comparing Clustering Performance}. For comparison, we use the widely utilized Silhouette score \citep{ROUSSEEUW198753} which lies between $[-1,1]$, with higher scores indicating better clustering performance. We show the results in Figure 1 for each combination setting considered. The fair clusters of Algorithm 3 used here are the same from Table 3. We observe that despite outperforming fair algorithms in terms of fairness, we still exhibit competitive clustering performance. We defer the results for the other performance metrics to the appendix (Section D.2), since those are unbounded and harder to interpret.

 %\vspace{-0.5cm}
% \subsection{Limitations of Proposed Algorithms}
 
  %\begin{wrapfigure}{R}{.5\textwidth}
\begin{figure*}[ht!]
\centering
\begin{subfigure}{.33\textwidth} %.32
  \centering
    \includegraphics[scale=0.09]{imgs/Bera_new.pdf}%0.09
  \caption{Combination \#1}
\smallskip
\end{subfigure}\hfill
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[scale=0.09]{imgs/Ghadiri_new.pdf}%
\caption{Combination \#2}
\smallskip
\end{subfigure}\hfill
\begin{subfigure}{.33\textwidth}
  \centering
    \includegraphics[scale=0.09]{imgs/Kleindessner_new.pdf}%0.1 scale
  \caption{Combination \#3}
\smallskip
\end{subfigure}
\caption{Comparing clustering performance of Algorithm 3 with fair clustering algorithms using Silhouette scores. (Higher scores indicate better clustering performance. As can be observed, fair clusters obtained via Algorithm 3 achieve similar clustering performance to SOTA algorithms, while providing improved fairness.)}
%\end{wrapfigure}
\end{figure*}

==> scratch.tex <==
%%SECTION 4.1
\iffalse
\begin{algorithm}
\caption{Proposed Algorithm for General $\mathcal{C}$ and $\mathcal{F}$}\label{sre}
\textbf{Input:} $U, \mathcal{C}, \mathcal{F}, \mathcal{A}, V_s, n', \xi$\\
\textbf{Output:} $V$
 \begin{algorithmic}[1]
 \Function{$f$}{$U, V, \mathcal{C}, \mathcal{F}$}
    \State $\mu \leftarrow \mathcal{C}(U \cup V)$
    \State \textbf{return} $\mathcal{F}(\mu, U)$
 \EndFunction
 \Statex
 \While{$\mathcal{F}(\mu, U) > \alpha$}
 \State \textbf{initialize} $V$ randomly with $|V| = V_s$
 \State \textbf{optimize} $V$ using \texttt{SRE}($n', f(U, V, \mathcal{C}, \mathcal{F}), \mathcal{A}$) 
 \State \textbf{obtain} optimized $V$ and $\mathcal{F}(\mu, U)$ as output from \texttt{SRE} and $\mathcal{A}$
 \State \textbf{if} $\mathcal{F}(\mu, U) \leq \alpha$ \textbf{return} $V$ \textbf{else} $V_s \leftarrow V_s + \xi$
 \EndWhile
 \end{algorithmic}
\end{algorithm}
\fi

Due to the blackbox and general nature of this setting, it is hard to give theoretical results about convergence and optimality. However, in the following subsections, when we can make some restrictive assumptions about $\mathcal{C}$ and $\mathcal{F}$, we provide more theoretical justification for our approaches. Furthermore, in our experiments on real-world data and in practice, we find that we can achieve improved fairness using Algorithm \ref{sre} with relative ease.


%%%SECTION 4.2

In this setting, we assume that both $\mathcal{C}$ and $\mathcal{F}$ are convex functions. This allows us to model the bi-level problem P1 much more easily since we know that a global optimum exists for the lower-level clustering problem. We now describe the standard approach for reducing the bi-level problem to a single-level optimization problem which is easier to solve:
\begin{enumerate}
    \item Derive the Karush-Kuhn-Tucker (KKT) conditions for the lower-level problem in P1.
    \item Replace the lower-level problem with the KKT conditions as constraints for the upper-level problem.
    \item Solving the obtained single-level problem is equivalent to solving P1.
\end{enumerate}

To extrapolate on the above approach for this setting, we can consider a convex clustering objective $\mathcal{C}$ and a convex $\mathcal{F}$. We can see that the social fairness cost $ \mathcal{F}_{\textrm{social}}$ is convex so we will consider that as our fairness notion. For $\mathcal{C}$, we consider a convex clustering objective called sum-of-norms (SON) clustering \citep{son, son-hier, son-kme, jiang2020identifying}. The SON clustering objective is strictly convex, and has been shown to be a relaxation for both k-means \citep{son-kme} and hierarchical clustering \citep{son-hier} approaches. The clustering objective is as follows:
\begin{equation}\tag{P2}
    \mathcal{C}_{\textrm{SON}}(U) \coloneqq \mu = \argmin_{\mu' \in \mathbb{R}^{n \times d}} \frac{1}{2}\sum_{j=1}^n||U_j - \mu_j'||^2 + \lambda\sum_{i<j}||\mu_i' - \mu_j'||
\end{equation}

Here the first term refers to a minimization between points and centers, and the second is a regularization term controlled by $\lambda$ to avoid trivial solutions. Moreover, we can have some $k$ centers by appropriate selection of $\lambda$ but due to how the objective is structured, we let $\mu \in \mathbb{R}^{n \times d}$. That is, some points will have the same centers and there will only be $k$ unique centers in $\mu$. 

We also borrow some ideas from \citep{Sun2021ConvexCM} which will allow us to derive the KKT conditions. Firstly, it is easier to model the regularization term if we create an ordering of all $(\mu_i, \mu_j)$ pairs that follow that $i < j$. Also, we can let each of the $n$ centers $\mu_i$ be a node in a graph $G$. Then, the ordering we have created, essentially enumerates the list of edges $E$ for the graph $G$. We denote this ordering as $O$ where we will have $|E| = |O|$. We also denote the node-arc-incidence matrix \citep{node-arc} for $(G, E)$ as $J \in \mathbb{R}^{n \times |O|}$. Using these, we can rewrite the objective in P2 as (where $\eta \in \mathbb{R}^{d \times |O|}$ is an auxiliary parameter):

\begin{equation}\tag{P3}
 \begin{aligned}
\min_{\mu, \eta} \quad & \frac{1}{2} ||\mu - U||^2 + \lambda \sum_{i \in O}||\eta^i||\\
\textrm{s.t.} \quad &  \mu^{T}J - \eta = 0\\
\end{aligned}   
\end{equation}

We can now also define the dual of problem P3 using the parameters $\theta \in \mathbb{R}^{d \times n}$ and $\zeta \in \mathbb{R}^{d \times |O|}$:


\begin{equation}\tag{P4}
 \begin{aligned}
\max_{\theta, \zeta} \quad &  \langle U^T, \theta \rangle - \frac{1}{2}||\theta||^2\\
\textrm{s.t.} \quad &  \zeta J^T - \theta = 0\\
& ||\zeta_i|| \leq \lambda, \forall i \in O\\
\end{aligned}   
\end{equation}


The KKT conditions for P3 and P4 are as follows (where prox(.) refers to the proximal operator of the Euclidean norm):
\begin{equation}\tag{KKT}
\begin{aligned}
    & \theta + \mu - U = 0\\
    & \eta - \textrm{prox}(\eta + \zeta) = 0\\
     & \mu^{T}J - \eta = 0\\
     & \zeta J^T - \theta = 0\\
\end{aligned} 
\end{equation}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this setting, we assume that both $\mathcal{C}$ and $\mathcal{F}$ are convex functions. We derive a negative result regarding the use of antidote data in this case, and for completeness, provide algorithms that compute fair centers as well. In particular, no other work has looked at convex clustering objectives from a fairness perspective, so ours is also the first work to do so. For any arbitrary $\mathcal{C}$ and $\mathcal{F}$ that are convex in $\mu$ we find that we can solve the bi-level problem and obtain the global optima without adding any antidote data. This is summarized in the following result:

\begin{claim}\label{no_antidote}
\textit{If $\mu^*$ is the optimal set of fair centers for problem \ref{p1} where both the clustering objective $\mathcal{C}$ and fairness cost $\mathcal{F}$ are convex functions, then an algorithm exists that obtains $\mu^*$ with $V$ set to $\emptyset$.}
\end{claim}

Effectively, if we consider solving problem \ref{p1} with $V \leftarrow \emptyset$, it reduces to solving problem \ref{p1.r} with $V \leftarrow \emptyset$. If $\mathcal{C}$ and $\mathcal{F}$ are convex in $\mu$ then Claim \ref{no_antidote} holds, and we can obtain the optimal center set $\mu^*$. If $\mathcal{F}(\mu^*, U) \leq \alpha$ then problem \ref{p1} is infeasible, otherwise we have found the optimal solution. We now discuss approaches towards solving the aforementioned problem.

\textbf{A standard first approach.} A simple approach towards solving the problem is to perform a single-level reduction from the bi-level form. This can be done by replacing the lower-level problem with its Karush-Kuhn-Tucker optimality conditions as constraints for the upper-level problem \citep{sinha2017review}. However, the obtained single-level optimization problem can now be non-convex, since the complementarity KKT condition can be non-convex. One would have to employ a non-convex solver for this problem, and in doing so, only locally optimal solutions are guaranteed. We thus give an improved approach based on bi-level subgradient descent, with strong theoretical guarantees of convergence to the globally optimal solution. 

\textbf{Subgradient descent based approach.} Since both the upper-level and lower-level problems are convex, we can utilize the subgradients of each function to optimize the overall bi-level problem. We first present our simple algorithm as Algorithm 

\begin{algorithm}
\caption{Proposed Algorithm for Convex $\mathcal{C}$ and $\mathcal{F}$}\label{cvx}
\textbf{Input:} \\
\textbf{Output:} 
 \begin{algorithmic}[1]
 \end{algorithmic}
\end{algorithm}
